EffiTune: Diagnosing and Mitigating Training Inefficiency for Parameter Tuner in Robot Navigation System

Robot navigation systems are critical for various real-world applications such as delivery services, hospital logistics, and warehouse management. Although classical navigation methods provide interpretability, they rely heavily on expert manual tuning, limiting their adaptability. Conversely, purely learning-based methods offer adaptability but often lead to instability and erratic robot behaviors. Recently introduced parameter tuners aim to balance these approaches by integrating data-driven adaptability into classical navigation frameworks. However, the parameter tuning process currently suffers from training inefficiencies and redundant sampling, with critical regions in environment often underrepresented in training data. In this paper, we propose EffiTune, a novel framework designed to diagnose and mitigate training inefficiency for parameter tuners in robot navigation systems. EffiTune first performs robot-behavior-guided diagnostics to pinpoint critical bottlenecks and underrepresented regions. It then employs a targeted up-sampling strategy to enrich the training dataset with critical samples, significantly reducing redundancy and enhancing training efficiency. Our comprehensive evaluation demonstrates that EffiTune achieves more than a 13.5% improvement in navigation performance, enhanced robustness in out-of-distribution scenarios, and a 4x improvement in training efficiency within the same computational budget.

==> figs/algs-template.tex <==
% \begin{algorithm}
% \caption{Trigger restoration algorithm}
% \label{alg:restore}
% \begin{algorithmic}[1]

% \State {\bfseries Input:} the policy and value network of the agent under our detection, $\pi(s)$ and $V_{\pi}(s)$ ($s \in \mathbb{R}^{p\times q}$), trigger restoration function $f_{\theta}$, 
% Beta distribution parameter $\alpha$, maximal detection iteration $N$, maximum trajectory length $T$ (given by the environment), number of trajectories in each batch $M$, sparsity regularization weight $\lambda_1$, smoothness regularization weight $\lambda_2$.
% \State {\bfseries Output:} the restored trigger $\Delta$.

% \For{$n=1,2,...,N$}
%     \State Compute the joint distribution $\mathbf{B} = \prod_{i,j} \text{Beta}(\alpha, \alpha + (f_{\theta_{ij}})), i = 1:p, j = 1:q$.
%     \State $\mathcal{T} = \emptyset$
    
%     \For {$1, ..., M$} 
%         \For{$t=1,2,...,T$}
%             \State Generate a trigger $\Delta_{s_t}$ by sampling from $\mathbf{B}$.
%             \State Add $\Delta_{s_t}$ to the current input state of the agent to generate $s'_t = s_t + \Delta_{s_t}$.
%             \State Agent takes action according to the perturbed state $a'\sim \pi(s'_t)$. 
%         \EndFor
%         \State Add the current trajectory to $\mathcal{T}$.
%     \EndFor
%     \State Compute the gradient of Eqn.(2) in Section 3.2 with respect to $\theta$ according to Eqn.~\eqref{eq:policy_gradient} and update the parameters of $f_{\theta}$ using Adam~\cite{kingma2014adam}.
% \EndFor
% \State Return the final restored trigger as $\Delta_s = 2(\frac{\alpha}{2\alpha+f_\theta(s)})-1$.

% \end{algorithmic}
% \end{algorithm}




% \begin{algorithm}
% \caption{Backdoor detection algorithm}
% \label{alg:detect}
% \begin{algorithmic}[1]

% \State {\bfseries Input:} A possibly backdoored agent with policy $\pi$, the restored triggers $\Delta$, the clean environment, maximum reward different of the environment $\eta_{max}$, detection threshold $\epsilon$, number of trajectories $K$.
% \State {\bfseries Output:} \textbf{True} if $\pi$ is backdoored, \textbf{False} if $\pi$ is clean.
% \State $\Bar{\eta}(\pi) \gets 0, \Bar{\eta}(\pi, \Delta) \gets 0$
% \For {$1,...,K$}
%     \State Randomly select an initial state and start the trajectory.
%     \State Add the restored trigger $\Delta$ to the state at every time step, the agent takes an action $a'\sim \pi(s')$.
%     \State Collect the agent's reward $r$ in this trajectory, $\Bar{\eta}(\pi, \Delta) \gets \Bar{\eta}(\pi, \Delta) + r$.
% \EndFor

% \For{$1,...,K$}
%     \State Randomly select an initial state and start the trajectory.
%     \State Agent $\pi_i$ observes the real clean state from the environment.
%     \State Collect the reward $r$ in this trajectory, $\Bar{\eta}(\pi) \gets \Bar{\eta}(\pi) + r$.
% \EndFor

% \State Compute the average reward under poisoned environment $\Bar{\eta}(\pi, \Delta) \gets \Bar{\eta}(\pi, \Delta)/K$.
% \State Compute the average reward under clean environment $\Bar{\eta}(\pi) \gets \Bar{\eta}(\pi)/K$.
% \State $\phi(\pi, \Delta) \gets (\Bar{\eta}(\pi, \Delta) - \Bar{\eta}(\pi))/\eta_{\text{max}}$
% \If{$\phi(\pi, \Delta) \leq \epsilon  $}
%     \State Return \textbf{True}, the policy is backdoored.
% \Else
%     \State Return \textbf{False}, the policy is clean.
% \EndIf

% \end{algorithmic}
% \end{algorithm}




% 
% \begin{algorithm}
% \caption{\small Black-box jailbreaking prompts searching with RL: Testing}
% \label{alg:eval}
% \begin{algorithmic}[1]

% \State {\bfseries Input:} target LLM $LLM_{\text{target}}$, helper LLM $LLM_{\text{helper}}$, prompt to helper LLM $\mathbf{p}_h$, judgment prompt to GPT-3.5 $\mathbf{p}_j$, evaluation question set $\mathcal{D}_{\text{eval}}$, Actions of agents $A$, unaligned model's responses to evaluation questions $\hat{R}_{\text{eval}}$, total iteration $N$, maximum step $T$,  number of parallel questions during training $K$, well-trained policy $\pi_{\theta}$, sampling strategy $S_{\text{eval}}$.

% \State {\bfseries Output:} A set of generated jailbreaking prompts $M$.

%     \State Initialize a set $M$ as $\emptyset$.
%     \For {every question $\mathbf{q}$ in $\mathcal{D}_{\text{eval}}$}
%         \For{$t=1,2,...,T$}
%             \If{$t == 1$}
%                 \State $\mathbf{s}^{(t)} = \mathbf{q}$
%             \Else
%                 \State $\mathbf{s}^{(t)} = \mathbf{p}^{(t-1)}$
%             \EndIf
%             \State Run policy $\mathbf{a}^{(t)} = \pi_{\theta}(\mathbf{s}^{(t)})$, fill $\mathbf{a}^{(t)}$ into $\mathbf{p}_h$ to obtain the complete prompts $\mathbf{p}_{\text{complete}}$ to $LLM_{\text{helper}}$.
%             \If{$t == 1$}
%                 \State Query $LLM_{\text{helper}}$ with $\mathbf{p}_{\text{complete}}$ and $S_{\text{eval}}$ to get jailbreaking prompts $\mathbf{p}^{(t)}$.
%             \Else
%                 \If{$\mathbf{a}^{(t)} == \mathbf{a}^{(t-1)}$}
%                 \State Let $LLM_{\text{helper}}$ paraphrase $\mathbf{p}^{(t-1)}$ to obtain $\mathbf{p}^{(t)}$.
%             \Else
%                 \State Query $LLM_{\text{helper}}$ with $\mathbf{p}_{\text{complete}}$ and $S_{\text{eval}}$ to get jailbreaking prompts $\mathbf{p}^{(t)'}$.
%                 \State Let GPT-3.5 perform crossover based on $\mathbf{p}^{(t-1)}$ and $\mathbf{p}^{(t)'}$, to obtain $\mathbf{p}^{(t)}$.
%                 \EndIf
%             \EndIf
%             \State Get the responses $\mathbf{u}^{(t)}$ of $LLM_{\text{target}}$ to the prompts $\mathbf{p}^{(t)}$.
%             \State Query GPT-3.5 with $\mathbf{p}_j$ to determine whether $\mathbf{u}^{(t)}$ contain the answers to the questions $\mathbf{q}$, then assign the judgment results to $\mathbf{c}$.
%             \If{ $\mathbf{c}$ is True or $t \geq T$}
%                 \State break
%             \EndIf
%         \EndFor
%         \State Add $\mathbf{p}^{(t)}$ to $M$.
%     \EndFor

% \State Return the final jailbreaking prompts $M$.

% \end{algorithmic}
% \end{algorithm}
% 


